Automated Detection of Double Nuclei Galaxies using GOTHIC and the Discovery of a Large Sample of Dual AGN

We present a novel algorithm to detect double nuclei galaxies (DNG) called GOTHIC (Graph BOosted iterated HIll Climbing) - that detects whether a given image of a galaxy has two or more closely separated nuclei. Our aim is to detect samples of dual or multiple active galactic nuclei (AGN) in galaxies. Although galaxy mergers are common, the detection of dual AGN is rare. Their detection is very important as they help us understand the formation of supermassive black hole (SMBH) binaries, SMBH growth and AGN feedback effects in multiple nuclei systems. There is thus a need for an algorithm to do a systematic survey of existing imaging data for the discovery of DNGs and dual AGN. We have tested GOTHIC on a known sample of DNGs and subsequently applied it to a sample of a million SDSS DR16 galaxies lying in the redshift range of 0 to 0.75 approximately, and have available spectroscopic data. We have detected 159 dual AGN in this sample, of which 2 are triple AGN systems. Our results show that dual AGN are not common, and triple AGN even rarer. The color (u-r) magnitude plots of the DNGs indicate that star formation is quenched as the nuclei come closer and as the AGN fraction increases. The quenching is especially prominent for dual/triple AGN galaxies that lie in the extreme end of the red sequence.

==> Tables/alldng.tex <==
\begin{longtable}{|p{0.2cm} c c c ccccc x{2.7cm}|}
% \centering
\caption{DAGN sources}
\label{table:DAGN}
%
%\hline
\\ \hline
No. & \begin{tabular}[c]{@{}l@{}}Co. \\ No.\end{tabular} & \begin{tabular}[c]{@{}c@{}}obj\\ ID\end{tabular} & \begin{tabular}[c]{@{}c@{}}Z\end{tabular} & g & r & \begin{tabular}[c]{@{}c@{}}Class \\ (SDSS) \end{tabular}& \begin{tabular}[c]{@{}c@{}}Subclass \\ (SDSS) \end{tabular}& \begin{tabular}[c]{@{}c@{}}Class\\ (From BPT)\end{tabular} & Comments \\
\hline
\hline
\multirow{2}{*}{1}  & 1 & 1237650762394959890 & 0.081 & 16.61 & 15.65 & GALAXY & BROADLINE & seyfert & \multirow{2}{*}{...}  \\
 & 2 & 1237650762394959891 & 0.081 & 17.74 & 16.83  & GALAXY & ... & composite &   \\
                     \hline
\multirow{2}{*}{2} & 1 & 1237651250964004981 & 0.102 & 18.54 & 17.51  & GALAXY & STARFORMING & composite & \multirow{2}{*}{...} \\
 & 2 & 1237651250964004982 & 0.102 & 18.28 & 17.48 & GALAXY & STARBURST & composite &  \\
  \hline
\multirow{2}{*}{3} & 1 & 1237651252018151484 & 0.075 & 16.48 & 15.53 & GALAXY & ... & composite & \multirow{2}{*}{...}  \\
 & 2 & 1237651252018151487 & 0.075  & 17.12 & 16.17 & GALAXY & ... & LINER &  \\
\hline
\multirow{2}{*}{4} & 1 & 1237651252024377492 & 0.089  & 17.59 & 16.62 & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237651252024377493 & 0.089 & 17.77 & 16.8 & GALAXY & ... & LINER &  \\
\hline
\multirow{2}{*}{5} & 1 & 1237651273510289469 & 0.118 & 16.79 & 15.75 & GALAXY & ... & LINER &\multirow{2}{*}{...}  \\
 & 2 & 1237651273510289470 & 0.119 & 19.02 & 17.93 & GALAXY & ... & composite &  \\
 \hline
\multirow{2}{*}{6} & 1 & 1237652600110383327 & 0.166 & 18.2 & 17.91 & GALAXY & STARFORMING & composite & \multirow{2}{*}{...}  \\
 & 2 & 1237652600110383328 & 0.166 & 18.53 & 17.75 & GALAXY & ... & seyfert &  \\
 \hline
 \multirow{2}{*}{7} & 1 & 1237652900234133595 & 0.2  & 19.19 & 17.74 & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237652900234133596 & 0.198 & 20.15 & 19.1 & GALAXY & STARFORMING & composite &  \\
 \hline
 \multirow{2}{*}{8} & 1 & 1237652946379604015 & 0.166 & 18.87 & 17.77 & GALAXY & ... & composite & \multirow{2}{*}{...} \\
 & 2 & 1237652946379604014 & 0.164 & 18.06 & 16.83  & GALAXY & ... & LINER &  \\
 \hline
 \multirow{2}{*}{9} & 1 & 1237653441374453924 & 0.069 & 17.21 & 16.3  & GALAXY & STARFORMING & composite &  \multirow{2}{*}{...} \\
 & 2 & 1237653441374453925 & 0.071 & 16.68 & 15.71  & GALAXY & ... & composite &  \\
 \hline
 \multirow{2}{*}{10} & 1 & 1237654031400566817 & 0.04 & 15.89 & 15.05 & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237654031400566818 & 0.04 & 16.2 & 15.32 & GALAXY & STARFORMING & composite &  \\
 \hline
 \multirow{2}{*}{11} & 1 & 1237654382516240489 & 0.125 & 17.32 & 16.16  & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237654382516240490 & 0.123 & 17.97 & 16.98 & GALAXY & ... & seyfert &  \\
 \hline
 \multirow{2}{*}{12} & 1 & 1237654880736968887 & 0.098 & 17.95 & 16.98  & GALAXY & ... & composite & \multirow{2}{*}{...} \\
 & 2 & 1237654880736968888 & 0.098 & 18.02 & 17.33  & GALAXY & STARFORMING & composite &  \\
 \hline
 \multirow{2}{*}{13} & 1 & 1237655106765521018 & 0.114 & 17.3 & 16.26 & GALAXY & ... & composite & \multirow{2}{*}{...} \\
 & 2 & 1237655106765521019 & 0.113 & 18.67 & 17.82 & GALAXY & ... & composite &  \\
 \hline
 \multirow{2}{*}{14} & 1 & 1237655369279733929 & 0.073 & 17.8 & 16.98  & GALAXY & STARFORMING & composite & \multirow{2}{*}{...} \\
 & 2 & 1237655369279733928 & 0.074 & 16.85 & 16.07  & GALAXY & STARFORMING & composite &  \\
 \hline
 \multirow{2}{*}{15} & 1 & 1237655465384214778 & 0.074 & 16.01 & 15.07 & GALAXY & ... & composite & \multirow{2}{*}{...}  \\
 & 2 & 1237655465384214780 & 0.071  & 18.11 & 17.19  & GALAXY & ... & composite &  \\
 \hline
 \multirow{2}{*}{16} & 1 & 1237655465920364786 & 0.098 & 18.02 & 17.06  & GALAXY & ... & seyfert & \multirow{2}{*}{...} \\
 & 2 & 1237655465920364787 & 0.098 & 18.98 & 18.04 & GALAXY & ... & composite &  \\
 \hline
 \multirow{2}{*}{17} & 1 & 1237655495979106559 & 0.091  & 18.24 & 17.34  & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237655495979106560 & 0.09 & 18.01 & 17.03  & GALAXY & STARFORMING & composite &  \\
 \hline
 \multirow{2}{*}{18}  & 1 & 1237655692474515647 & 0.175  & 17.94 & 16.58 & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237655692474515648 & 0.174 & 18.99 & 17.86  & GALAXY & ... & composite &  \\
 \hline
 \multirow{2}{*}{19}& 1 & 1237656239009104192 & 0.134 & 18.57 & 17.51 & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237656239009104193 & 0.133 & 18.5 & 17.29  & GALAXY & ... & LINER &  \\
 \hline
\multirow{2}{*}{20} & 1 & 1237656567582294307 & 0.027  & 16.53 & 15.54 & GALAXY & ... & composite & \multirow{2}{*}{...} \\
 & 2 & 1237656567582294308 & 0.026  & 17.06 & 16.24 & GALAXY & ... & composite &  \\
 \hline
 \multirow{2}{*}{21} & 1 & 1237667253455356213 & 0.09  & 16.54 & 15.45 & GALAXY & ... & composite & \multirow{2}{*}{...} \\
 & 2 & 1237667253455356214 & 0.091 & 20.2 & 19.36  & GALAXY & ... & LINER &  \\
 \hline
 \multirow{2}{*}{22} & 1 & 1237656567585833094 & 0.057  & 15.92 & 14.97 & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237656567585833097 & 0.057 & 17.11 & 15.8  & GALAXY & ... & seyfert &  \\
 \hline
 \multirow{2}{*}{23} & 1 & 1237656906354393114 & 0.023  & 14.84 & 14.01 & GALAXY & ... & LINER & \multirow{2}{*}{...}  \\
 & 2 & 1237656906354393115 & 0.024 & 20.86 & 20.73  & GALAXY & STARFORMING & composite &  \\
 \hline
 \multirow{2}{*}{24} & 1 & 1237657189817516083 & 0.139  & 18.87 & 17.63 & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237657189817516085 & 0.138 & 19.38 & 18.3 & GALAXY & ... & composite &  \\
 \hline
\multirow{2}{*}{25} & 1 & 1237657221485625353 & 0.046  & 15.08 & 14.24 & GALAXY & BROADLINE & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237657221485559856 & 0.046 & 17.52 & 16.67 & GALAXY & ... & LINER &  \\
 \hline
\multirow{2}{*}{26} & 1 & 1237657609104982532 & 0.153 & 18.17 & 17.06 & GALAXY & ... & seyfert & \multirow{2}{*}{...} \\
 & 2 & 1237657609104982533 & 0.153  & 19.09 & 17.89 & GALAXY & ... & LINER &  \\
\hline
\multirow{2}{*}{27} & 1 & 1237657612874940605 & 0.07  & 17.27 & 16.32 & GALAXY & ... & composite & \multirow{2}{*}{...}  \\
 & 2 & 1237657612874940607 & 0.069  & 18.41 & 17.55 & GALAXY & ... & composite &  \\
\hline
\multirow{2}{*}{28} & 1 & 1237657628432531602 & 0.078  & 16.75 & 15.74  & GALAXY & BROADLINE & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237657628432531603 & 0.078 & 18.11 & 17.13 & GALAXY & ... & composite &  \\
\hline
\multirow{2}{*}{29} & 1 & 1237657857148911724 & 0.06 & 17.54 & 16.73 & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237657857148911725 & 0.06  & 16.83 & 16 & GALAXY & ... & composite &  \\
\hline
\multirow{2}{*}{30} & 1 & 1237658300056338796 & 0.139 & 17.24 & 16.34 & GALAXY & STARFORMING & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237658300056338797 & 0.138 & 17.93 & 16.99 & GALAXY & ... & composite &  \\
 \hline
\multirow{2}{*}{31} & 1 & 1237658424090493080 & 0.072  & 17.56 & 16.62 & GALAXY & STARFORMING & composite & \multirow{2}{*}{...} \\
 & 2 & 1237658424090493081 & 0.071  & 17.17 & 16.23 & GALAXY & ... & composite &  \\
\hline
\multirow{2}{*}{32} & 1 & 1237658611440222364 & 0.144  & 18.18 & 16.99  & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237658611440222365 & 0.145  & 18.7 & 17.62 & GALAXY & ... & composite &  \\
\hline
\multirow{2}{*}{33} & 1 & 1237658918533005504 & 0.113  & 18.26 & 17.27  & GALAXY & ... & seyfert & \multirow{2}{*}{...} \\
 & 2 & 1237658918533005505 & 0.113  & 18.78 & 17.87  & GALAXY & ... & composite &  \\
\hline
\multirow{2}{*}{34} & 1 & 1237659119862939753 & 0.144  & 17.32 & 16.44  & GALAXY & STARFORMING & composite & \multirow{2}{*}{...} \\
 & 2 & 1237659119862939754 & 0.145  & 18.47 & 17.18  & GALAXY & ... & seyfert &  \\
\hline
\multirow{2}{*}{35} & 1 & 1237659119864774675 & 0.099  & 16.98 & 15.84  & GALAXY & ... & composite & \multirow{2}{*}{...}  \\
 & 2 & 1237659119864774676 & 0.1  & 18.46 & 17.43  & GALAXY & ... & seyfert &  \\
\hline
\multirow{2}{*}{36} & 1 & 1237659132206448648 & 0.11  & 18.89 & 17.87  & GALAXY & ... & seyfert & \multirow{2}{*}{...} \\
 & 2 & 1237659132206448651 & 0.11  & 19.81 & 18.81  & GALAXY & ... & seyfert &  \\
\hline
\multirow{2}{*}{37} & 1 & 1237660240313385134 & 0.142  & 19.36 & 18.23 & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237660240313385135 & 0.142  & 18.66 & 17.75  & GALAXY & STARFORMING & composite &  \\
\hline
\multirow{2}{*}{38} & 1 & 1237660240313712760 & 0.038  & 15.09 & 14.22  & GALAXY & STARFORMING & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237660240313712761 & 0.038  & 19.4 & 18.63  & GALAXY & ... & composite &  \\
\hline
\multirow{2}{*}{39} & 1 & 1237660241385029806 & 0.074  & 17.26 & 16.32  & GALAXY & BROADLINE & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237660241385029810 & 0.073  & 18.49 & 17.54  & GALAXY & ... & composite &  \\
\hline
\multirow{2}{*}{40} & 1 & 1237660669282812044 & 0.115  & 18.74 & 17.73 & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237660669282812045 & 0.116  & 18.87 & 17.85  & GALAXY & ... & seyfert &  \\
\hline
\multirow{2}{*}{41} & 1 & 1237660963472932915 & 0.048  & 16.06 & 15.01  & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237660963472932916 & 0.048 & 16.39 & 15.57 & GALAXY & STARFORMING & composite &  \\
\hline
\multirow{2}{*}{42} & 1 & 1237661086415585604 & 0.047  & 14 & 13.14  & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237661086415585607 & 0.048  & 17.66 & 15.61  & GALAXY & ... & composite &  \\
\hline
\multirow{2}{*}{43} & 1 & 1237661137963254106 & 0.129  & 17.68 & 16.6  & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237661137963254107 & 0.129  & 18.95 & 17.83  & GALAXY & ... & LINER &  \\
\hline
\multirow{2}{*}{44} & 1 & 1237661151377424586 & 0.104  & 17.78 & 16.58  & GALAXY & ... & composite & \multirow{2}{*}{...} \\
 & 2 & 1237661151377424587 & 0.104  & 18.62 & 17.73  & GALAXY & ... & seyfert &  \\
\hline
\multirow{2}{*}{45} & 1 & 1237661352706179107 & 0.082  & 16.61 & 15.82  & GALAXY & ... & composite & \multirow{2}{*}{...} \\
 & 2 & 1237661352706179108 & 0.082  & 17.79 & 16.8  & GALAXY & ... & composite &  \\
\hline
\multirow{2}{*}{46} & 1 & 1237661382778093715 & 0.069  & 16.2 & 15.3  & GALAXY & ... & composite & \multirow{2}{*}{...} \\
 & 2 & 1237661382778093716 & 0.068  & 16.93 & 16.04  & GALAXY & BROADLINE & composite &  \\
\hline
\multirow{2}{*}{47} & 1 & 1237661418748444829 & 0.107  & 17.06 & 16.09  & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237661418748444830 & 0.107  & 17.91 & 16.95  & GALAXY & ... & seyfert &  \\
\hline
\multirow{2}{*}{48} & 1 & 1237661812274233471 & 0.064 & 16.26 & 15.59  & GALAXY & STARBURST & composite & \multirow{2}{*}{...} \\
 & 2 & 1237661812274233472 & 0.064  & 17.36 & 16.41  & GALAXY & ... & LINER &  \\
\hline
\multirow{2}{*}{49} & 1 & 1237661813348106331 & 0.123  & 17.69 & 16.67  & GALAXY & ... & seyfert & \multirow{2}{*}{...} \\
 & 2 & 1237661813348106332 & 0.124  & 18.72 & 17.74  & GALAXY & ... & composite &  \\
\hline
\multirow{2}{*}{50} & 1 & 1237661850411204729 & 0.076  & 16.56 & 15.75  & GALAXY & STARFORMING & composite & \multirow{2}{*}{...} \\
 & 2 & 1237661850411204730 & 0.075 & 17.42 & 16.5   & GALAXY & ... & seyfert &  \\
\hline
\multirow{2}{*}{51} & 1 & 1237661871330361452 & 0.112  & 17.41 & 16.36  & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237661871330361453 & 0.112  & 16.78 & 15.77  & GALAXY & ... & composite &  \\
 \hline
\multirow{2}{*}{52} & 1 & 1237661957762842806 & 0.133  & 18.39 & 17.21  & GALAXY & ... & composite & \multirow{2}{*}{...} \\
 & 2 & 1237661957762842807 & 0.133  & 18.38 & 17.34  & GALAXY & ... & seyfert &  \\
\hline
\multirow{2}{*}{53} & 1 & 1237661966886633584 & 0.131  & 18.37 & 17.27 & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237661966886633585 & 0.131  & 18.68 & 17.6  & GALAXY & ... & LINER &  \\
\hline
\multirow{2}{*}{54} & 1 & 1237661971721945220 & 0.073  & 17.2 & 16.23  & GALAXY & ... & seyfert & \multirow{2}{*}{...} \\
 & 2 & 1237661971721945221 & 0.074  & 16.58 & 15.72  & GALAXY & ... & LINER &  \\
\hline
\multirow{2}{*}{55} & 1 & 1237662193453760669 & 0.171  & 18.79 & 17.6 & GALAXY & ... & composite & \multirow{2}{*}{...} \\
 & 2 & 1237662193453760670 & 0.173  & 18.82 & 17.62 & GALAXY & ... & seyfert &  \\
\hline
\multirow{2}{*}{56} & 1 & 1237662194541002843 & 0.073  & 16.41 & 15.47 & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237662194541002844 & 0.074  & 16.61 & 15.8 & GALAXY & ... & seyfert &  \\
\hline

\multirow{2}{*}{57} & 1 & 1237662198280552769 & 0.172  & 18.85 & 17.62 & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237662198280552768 & 0.172  & 18.94 & 17.69 & GALAXY & ... & LINER &  \\
\hline
\\
\\
\hline
\multirow{2}{*}{58} & 1 & 1237662225666932750 & 0.099  & 17.88 & 16.83  & GALAXY & ... & composite & \multirow{2}{*}{...} \\
 & 2 & 1237662225666932751 & 0.099  & 19.04 & 18.21  & GALAXY & ... & composite &  \\
\hline
\multirow{2}{*}{59} & 1 & 1237662335178178801 & 0.065  & 16.5 & 15.57 & GALAXY & ... & seyfert & \multirow{2}{*}{...} \\
 & 2 & 1237662335178178802 & 0.065  & 17.95 & 17.05  & GALAXY & ... & seyfert &  \\
\hline
\multirow{2}{*}{60} & 1 & 1237662336792920258 & 0.069 & 17.12 & 16.25  & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237662336792920257 & 0.07  & 16.53 & 15.67 & GALAXY & STARFORMING & composite &  \\
\hline
\multirow{2}{*}{61} & 1 & 1237662474231021741 & 0.117 & 17.17 & 16.09 & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237662474231021742 & 0.117 & 18.18 & 17.23  & GALAXY & ... & composite &  \\
\hline
\multirow{2}{*}{62} & 1 & 1237662498390737019 & 0.154 & 17.83 & 16.69  & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237662498390737020 & 0.153  & 18.12 & 16.95  & GALAXY & ... & LINER &  \\
\hline
\multirow{2}{*}{63} & 1 & 1237662200436752504 & 0.105 & 17.14 & 16.09 & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237662636375867758 & 0.105 & 17.9 & 16.8  & GALAXY & STARFORMING & composite &  \\
\hline
\multirow{2}{*}{64} & 1 & 1237662640123609565 & 0.059 & 16.41 & 15.48  & GALAXY & ... & composite & \multirow{2}{*}{...} \\
 & 2 & 1237662640123609566 & 0.06 & 22.5 & 21.75 & GALAXY & ... & composite &  \\
\hline
\multirow{2}{*}{65} & 1 & 1237663463145537628 & 0.084 & 14.96 & 13.92 & GALAXY & ... & seyfert & \multirow{2}{*}{...}  \\
 & 2 & 1237663463145537634 & 0.084  & 17.17 & 16.97 & GALAXY & ... & LINER &  \\
\hline
\multirow{2}{*}{66} & 1 & 1237663543683318057 & 0.084  & 17.98 & 17.1 & GALAXY & ... & composite & \multirow{2}{*}{...} \\
 & 2 & 1237663543683318058 & 0.085  & 18.68 & 17.93 & GALAXY & STARFORMING & composite &  \\
\hline
\multirow{2}{*}{67} & 1 & 1237663782589432032 & 0.139  & 18.93 & 17.8  & GALAXY & ... & composite & \multirow{2}{*}{...}  \\
 & 2 & 1237663782589432033 & 0.139  & 18.87 & 17.8  & GALAXY & ... & composite &  \\
\hline
\multirow{2}{*}{68} & 1 & 1237663783122370706 & 0.186  & 18.56 & 17.25 & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237663783122370707 & 0.183 & 19.95 & 18.77  & GALAXY & ... & LINER &  \\
\hline
\multirow{2}{*}{69} & 1 & 1237663783131283514 & 0.089 & 16.95 & 16.52 & GALAXY & STARBURST & composite & \multirow{2}{*}{...} \\
 & 2 & 1237663783131283515 & 0.089 & 17.46 & 16.59  & GALAXY & ... & composite &  \\
\hline
\multirow{2}{*}{70} & 1 & 1237663783136985126 & 0.12 & 18.76 & 17.85  & GALAXY & ... & composite & \multirow{2}{*}{...}  \\
 & 2 & 1237663783136985125 & 0.121 & 18.08 & 17.05  & GALAXY & ... & seyfert &  \\
\hline
\multirow{2}{*}{71} & 1 & 1237663783674183846 & 0.112  & 18.22 & 17.25  & GALAXY & STARFORMING & composite & \multirow{2}{*}{...} \\
 & 2 & 1237663783674183847 & 0.111  & 18.5 & 18.01 & GALAXY & STARFORMING & composite &  \\
\hline
\multirow{2}{*}{72} & 1 & 1237663784195653787 & 0.079 & 18.56 & 17.53  & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237663784195653788 & 0.079 & 18.15 & 17.67  & GALAXY & ... & composite &  \\
\hline
\multirow{2}{*}{73} & 1 & 1237663784200831188 & 0.073 & 17.56 & 16.65  & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237663784200831189 & 0.074 & 18.31 & 17.48  & GALAXY & STARFORMING & composite &  \\
\hline
\multirow{2}{*}{74} & 1 & 1237663784739995886 & 0.115 & 17.53 & 16.79  & GALAXY & STARFORMING & composite & \multirow{2}{*}{...} \\
 & 2 & 1237663784739995887 & 0.116 & 18.39 & 17.38  & GALAXY & ... & composite &  \\
\hline
\multirow{2}{*}{75} & 1 & 1237664291548823599 & 0.041  & 16.03 & 15.17  & GALAXY & BROADLINE & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237664291548823600 & 0.041 & 14.75 & 13.92  & GALAXY & ... & LINER &  \\
\hline
\multirow{2}{*}{76} & 1 & 1237664667352039631 & 0.084 & 18.05 & 17.08  & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237664667352039632 & 0.085 & 17.56 & 16.84  & GALAXY & STARFORMING & LINER &  \\
\hline
\multirow{2}{*}{77} & 1 & 1237664817676484746 & 0.215 & 18.67 & 17.79  & GALAXY & STARFORMING & composite & \multirow{2}{*}{...} \\
 & 2 & 1237664817676484748 & 0.216  & 18.88 & 17.84  & GALAXY & STARFORMING & composite &  \\
\hline
\multirow{2}{*}{78} & 1 & 1237664871900577858 & 0.049  & 17.32 & 16.45 & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237664871900577859 & 0.051 & 17.96 & 17.07  & GALAXY & ... & seyfert &  \\
\hline
\multirow{2}{*}{79} & 1 & 1237664877803077714 & 0.116 & 18.6 & 17.59  & GALAXY & ... & LINER & \multirow{2}{*}{...}  \\
 & 2 & 1237664877803077715 & 0.118 & 18.47 & 17.43  & GALAXY & ... & LINER &  \\
\hline
\multirow{2}{*}{80} & 1 & 1237664877807927453 & 0.206 & 19 & 17.68  & GALAXY & ... & seyfert &  \multirow{2}{*}{...}\\
 & 2 & 1237664877807927454 & 0.207 & 18.92 & 17.62  & GALAXY & ... & LINER &  \\
\hline
\multirow{2}{*}{81} & 1 & 1237665103283814519 & 0.075 & 17.47 & 16.54  & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237665103283814520 & 0.075  & 16.45 & 15.57 & GALAXY & ... & LINER &  \\
\hline
\multirow{2}{*}{82} & 1 & 1237665129610936526 & 0.154 & 18.7 & 17.56  & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237665129610936527 & 0.153 & 18.88 & 17.89  & GALAXY & STARFORMING & composite &  \\
\hline
\multirow{2}{*}{83} & 1 & 1237665328779100316 & 0.154 & 18.79 & 17.63  & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237665328779100317 & 0.155 & 18.15 & 16.98  & GALAXY & ... & seyfert &  \\
\hline
\multirow{2}{*}{84} & 1 & 1237665330927435873 & 0.088 & 17.43 & 16.48  & GALAXY & STARBURST & composite & \multirow{2}{*}{...} \\
 & 2 & 1237665330927435875 & 0.088 & 18.99 & 18.25 & GALAXY & ... & seyfert &  \\
\hline
\multirow{2}{*}{85} & 1 & 1237665331455459378 & 0.072 & 16.66 & 15.84  & GALAXY & STARFORMING & seyfert & \multirow{2}{*}{...} \\
 & 2 & 1237665331455459379 & 0.073 & 17.42 & 17.16  & GALAXY & STARFORMING & composite &  \\
\hline
\multirow{2}{*}{86} & 1 & 1237665331457425465 & 0.128 & 17.77 & 16.62  & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237665331457425466 & 0.127 & 18 & 16.8  & GALAXY & ... & LINER &  \\
\hline
\\
\\
\hline
\multirow{2}{*}{87} & 1 & 1237665428091240506 & 0.14  & 17.25 & 16.27 & GALAXY & ... & seyfert & \multirow{2}{*}{...} \\
 & 2 & 1237665428091240507 & 0.141  & 19.37 & 18.32  & GALAXY & ... & composite &  \\
\hline
\multirow{2}{*}{88} & 1 & 1237665429713780966 & 0.088  & 18.43 & 17.5  & GALAXY & ... & composite & \multirow{2}{*}{...} \\
 & 2 & 1237665429713846350 & 0.09 & 17.52 & 16.57  & GALAXY & ... & LINER &  \\
\hline
\multirow{2}{*}{89} & 1 & 1237665440439336990 & 0.065 & 15.47 & 14.57 & GALAXY & ... & composite & \multirow{2}{*}{...} \\
 & 2 & 1237665440439336991 & 0.061 & 15.71 & 14.82  & GALAXY & ... & LINER &  \\
\hline
\multirow{2}{*}{90} & 1 & 1237665531723579489 & 0.132 & 17.42 & 16.37  & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237665531723579490 & 0.13  & 18.17 & 17.16  & GALAXY & ... & LINER &  \\
\hline
\multirow{2}{*}{91} & 1 & 1237665566082269200 & 0.094 & 16.75 & 15.76  & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237665566082269201 & 0.094  & 18.19 & 17.2  & GALAXY & ... & composite &  \\
\hline
\multirow{2}{*}{92} & 1 & 1237666185634447638 & 0.121  & 18.79 & 17.64 & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237666185634447639 & 0.121  & 18.52 & 17.3  & GALAXY & ... & LINER &  \\
\hline
\multirow{2}{*}{93} & 1 & 1237666301627924604 & 0.156  & 20.86 & 19.58  & GALAXY & ... & composite & \multirow{2}{*}{...} \\
 & 2 & 1237666301627924605 & 0.156  & 17.89 & 16.97 & GALAXY & STARFORMING & LINER &  \\
\hline
\multirow{2}{*}{94} & 1 & 1237666407381598382 & 0.08  & 18.01 & 17.08 & GALAXY & STARFORMING & composite &  \multirow{2}{*}{...} \\
 & 2 & 1237666407381598383 & 0.08  & 16.91 & 16.49  & GALAXY & ... & composite &  \\
\hline
\multirow{2}{*}{95} & 1 & 1237667109574279383 & 0.201  & 18.89 & 17.51  & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237667109574279384 & 0.2  & 19.12 & 17.79  & GALAXY & ... & composite &  \\
\hline
\multirow{2}{*}{96} & 1 & 1237667209974710300 & 0.078  & 17.88 & 17.4  & GALAXY & STARBURST & composite & \multirow{2}{*}{...} \\
 & 2 & 1237667209974710301 & 0.078  & 17.72 & 16.83  & GALAXY & STARFORMING & composite &  \\
\hline
\multirow{2}{*}{97} & 1 & 1237667212115050866 & 0.172  & 18.79 & 17.51 & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237667212115050867 & 0.173  & 19.53 & 18.38  & GALAXY & ... & composite &  \\
\hline
\multirow{2}{*}{98} & 1 & 1237667212136284360 & 0.138  & 18.89 & 17.71 & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237667212136284359 & 0.13  & 17.88 & 17.03 & GALAXY & ... & seyfert &  \\
\hline
\multirow{2}{*}{99} & 1 & 1237667253453324693 & 0.141 & 17.65 & 16.64  & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237667253453324694 & 0.141  & 18.28 & 17.11 & GALAXY & ... & LINER &  \\
\hline
\multirow{2}{*}{100} & 1 & 1237667254546006103 & 0.145  & 18.31 & 17.88 & GALAXY & STARFORMING & composite & \multirow{2}{*}{...} \\
 & 2 & 1237667254546006104 & 0.145  & 18.64 & 17.84 & GALAXY & ... & LINER &  \\
\hline
\multirow{2}{*}{101} & 1 & 1237667323250213040 & 0.038  & 16.18 & 15.28 & GALAXY & STARFORMING & composite & \multirow{2}{*}{...}  \\
 & 2 & 1237667323250213041 & 0.038  & 18.34 & 18 & GALAXY & ... & composite &  \\
\hline
\multirow{2}{*}{102} & 1 & 1237667323796127885 & 0.083  & 17.01 & 16.18 & GALAXY & ... & LINER & \multirow{2}{*}{...}  \\
 & 2 & 1237667323796127886 & 0.083  & 18.27 & 17.47 & GALAXY & STARFORMING & composite &  \\
\hline
\multirow{2}{*}{103} & 1 & 1237667442437914759 & 0.079  & 17.58 & 16.64 & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237667442437914760 & 0.08  & 17.55 & 16.73  & GALAXY & STARFORMING & composite &  \\
\hline
\multirow{2}{*}{104} & 1 & 1237667549268148435 & 0.118  & 17.52 & 16.73  & GALAXY & STARFORMING & composite &  \multirow{2}{*}{...} \\
 & 2 & 1237667549268213959 & 0.116  & 17.25 & 16.43 & GALAXY & STARFORMING & composite &  \\
\hline
\multirow{2}{*}{105} & 1 & 1237667733989949671 & 0.09  & 18.33 & 17.36 & GALAXY & ... & composite & \multirow{2}{*}{...} \\
 & 2 & 1237667733989949676 & 0.089  & 18.26 & 17.31 & GALAXY & ... & seyfert &  \\
\hline
\multirow{2}{*}{106} & 1 & 1237667734526886197 & 0.119  & 18.69 & 17.65 & GALAXY & ... & composite & \multirow{2}{*}{...} \\
 & 2 & 1237667734526886198 & 0.118 & 18.11 & 17.08  & GALAXY & ... & seyfert &  \\
\hline
\multirow{2}{*}{107} & 1 & 1237667736133828618 & 0.096  & 16.91 & 15.97 & GALAXY & ... & seyfert & \multirow{2}{*}{...} \\
 & 2 & 1237667736133828619 & 0.097 & 17.06 & 16.07  & GALAXY & ... & LINER &  \\
\hline
\multirow{2}{*}{108} & 1 & 1237667781774934219 & 0.102 & 16.8 & 15.87  & GALAXY & ... & composite & \multirow{2}{*}{...} \\
 & 2 & 1237667781774934220 & 0.103 & 18.28 & 17.3 & GALAXY & ... & seyfert &  \\
\hline
\multirow{2}{*}{109} & 1 & 1237667783883817113 & 0.148 & 18.42 & 17.24 & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237667783883817114 & 0.149 & 18.71 & 17.55  & GALAXY & ... & seyfert &  \\
\hline
\multirow{2}{*}{110} & 1 & 1237667783929299179 & 0.051 & 15.52 & 14.64  & GALAXY & BROADLINE & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237667783929299180 & 0.05 & 16.51 & 15.66  & GALAXY & BROADLINE & LINER &  \\
\hline
\multirow{2}{*}{111} & 1 & 1237667910069190795 & 0.077  & 16.79 & 16.11 & GALAXY & STARFORMING & composite & \multirow{2}{*}{...}  \\
 & 2 & 1237667910069190796 & 0.077 & 16.94 & 16.16 & GALAXY & STARFORMING & composite &  \\
\hline
\multirow{2}{*}{112} & 1 & 1237667916494012508 & 0.066 & 16.64 & 15.76  & GALAXY & ... & seyfert & \multirow{2}{*}{...} \\
 & 2 & 1237667916494012509 & 0.065 & 16.66 & 15.76  & GALAXY & ... & LINER &  \\
\hline
\multirow{2}{*}{113} & 1 & 1237668271362211975 & 0.088 & 17.3 & 16.28  & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237668271362211976 & 0.089 & 17.94 & 17.1  & GALAXY & ... & LINER &  \\
\hline
\multirow{2}{*}{114} & 1 & 1237668298204446938 & 0.119 & 17.77 & 17.09  & GALAXY & STARBURST & composite & \multirow{2}{*}{...} \\
 & 2 & 1237668298204446939 & 0.119  & 17.98 & 16.93 & GALAXY & STARFORMING & composite &  \\
\hline

\multirow{2}{*}{115} & 1 & 1237668589722534078 & 0.153  & 18.66 & 17.59 & GALAXY & STARFORMING & composite & \multirow{2}{*}{...} \\
 & 2 & 1237668589722534074 & 0.152 & 19.15 & 17.98  & GALAXY & ... & composite &  \\
 \hline
 \\
 \\
\hline
\multirow{2}{*}{116} & 1 & 1237668623551103255 & 0.216  & 18.75 & 17.72  & GALAXY & ... & composite & \multirow{2}{*}{...} \\
 & 2 & 1237668623551103256 & 0.216 & 20.54 & 18.94  & GALAXY & ... & composite &  \\
\hline
\multirow{2}{*}{117} & 1 & 1237668672938115205 & 0.136  & 17.47 & 16.4 & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237668672938115206 & 0.135  & 18.91 & 17.89 & GALAXY & ... & composite &  \\
\hline
\multirow{2}{*}{118} & 1 & 1237670964313456852 & 0.076 & 16.11 & 15.16  & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237670964313456853 & 0.078 & 16.55 & 15.61 & GALAXY & ... & LINER &  \\
\hline
\multirow{2}{*}{119} & 1 & 1237670965383266430 & 0.031 & 15.93 & 15.04 & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237670965383266433 & 0.03 & 16.39 & 15.57  & GALAXY & ... & composite &  \\
\hline
\multirow{2}{*}{120} & 1 & 1237671931208925416 & 0.073  & 16.19 & 15.26 & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237671931208925417 & 0.073 & 17.76 & 16.78  & GALAXY & ... & LINER &  \\
\hline
\multirow{2}{*}{121} & 1 & 1237673807580693064 & 0.144  & 17.59 & 16.39 & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237673807580693069 & 0.14  & 18.43 & 17.37 & GALAXY & ... & composite &  \\
\hline
\multirow{2}{*}{122} & 1 & 1237673808116122327 & 0.1  & 16.93 & 16.19 & GALAXY & STARFORMING & composite & \multirow{2}{*}{...}  \\
 & 2 & 1237673808116122329 & 0.099  & 17.35 & 16.4  & GALAXY & ... & LINER &  \\
\hline
\multirow{2}{*}{123} & 1 & 1237674649921061067 & 0.096  & 17.12 & 16.11 & GALAXY & ... & composite & \multirow{2}{*}{...} \\
 & 2 & 1237674649921061068 & 0.093  & 17.3 & 16.32 & GALAXY & ... & composite &  \\
\hline
\multirow{2}{*}{124} & 1 & 1237657587096289353 & 0.025 & 14.72 & 13.89  & GALAXY & ... & seyfert & \multirow{2}{*}{...} \\
 & 2 & 1237657587096289354 & 0.025  & 18.77 & 18.21 & GALAXY & ... & seyfert &  \\
\hline
\multirow{2}{*}{125} & 1 & 1237666210341978625 & 0.06  & 17.66 & 16.97 & GALAXY & STARFORMING & composite & \multirow{2}{*}{...}  \\
 & 2 & 1237666210341978627 & 0.061 & 17.13 & 16.36  & GALAXY & STARFORMING & composite &  \\
\hline
\multirow{2}{*}{126} & 1 & 1237662335180341316 & 0.064  & 16.61 & 15.84 & GALAXY & STARFORMING & composite & \multirow{2}{*}{...}  \\
 & 2 & 1237662335180341327 & 0.064 & 21.32 & 21.88 & GALAXY & STARFORMING & composite &  \\
\hline
\multirow{2}{*}{127} & 1 & 1237659327092752463 & 0.149 & 18.12 & 17.52 & QSO & STARBURST & seyfert & \multirow{2}{*}{...}  \\
 & 2 & 1237659327092752464 & 0.15  & 18.58 & 17.62 & GALAXY & STARFORMING & composite &  \\
\hline
\multirow{2}{*}{128} & 1 & 1237667915957665832 & 0.065 & 15.74 & 14.74 & GALAXY & ... & composite & \multirow{2}{*}{...} \\
 & 2 & 1237667915957665835 & 0.065  & 16.17 & 15.24 & GALAXY & AGN & composite &  \\
\hline
\multirow{2}{*}{129} & 1 & 1237668588651282620 & 0.074  & 16.46 & 15.57 & GALAXY & ... & LINER &  \multirow{2}{*}{...} \\
 & 2 & 1237668588651282621 & 0.074 & 16.61 & 15.76  & GALAXY & AGN & LINER &  \\
\hline
\multirow{2}{*}{130} & 1 & 1237671262267506768 & 0.052  & 14.94 & 14.02  & GALAXY & AGN & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237671262267506767 & 0.053  & 17.55 & 16.73  & GALAXY & ... & LINER &  \\
\hline
\multirow{2}{*}{131} & 1 & 1237666227490586650 & 0.103 & 17.04 & 16.29  & GALAXY & STARBURST & composite & \multirow{2}{*}{...} \\
 & 2 & 1237666227490586649 & 0.104 & 18.98 & 17.95  & QSO & STARBURST & composite &  \\
\hline
\multirow{2}{*}{132} & 1 & 1237666228063371544 & 0.1 & 18.03 & 16.97  & GALAXY & AGN & seyfert & \multirow{2}{*}{...} \\
 & 2 & 1237666228063371545 & 0.099 & 16.91 & 16.08  & GALAXY & STARFORMING & composite &  \\
 \hline
\multirow{2}{*}{133} & 1 & 1237667252917895553 & 0.153 & 17.7 & 16.48  & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237667252917895554 & 0.156  & 17.78 & 16.94 & QSO & STARBURST & composite &  \\
\hline
\multirow{2}{*}{134} & 1 & 1237664667360755820 & 0.152 & 19.07 & 18.03 & QSO & STARBURST & composite & \multirow{2}{*}{...} \\
 & 2 & 1237664667360755822 & 0.153 & 19.56 & 19.29  & GALAXY & AGN & composite &  \\
\hline
\multirow{2}{*}{135} & 1 & 1237660240314433647 & 0.156  & 18.85 & 17.5 & GALAXY & ... & seyfert & \multirow{2}{*}{...} \\
 & 2 & 1237660240314433648 & 0.158 & 19.23 & 18.07  & GALAXY & AGN & seyfert &  \\
\hline
\multirow{2}{*}{136} & 1 & 1237655502962688659 & 0.03  & 15.96 & 15.16 & GALAXY & AGN & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237655502962688660 & 0.029  & 19.28 & 18.1 & GALAXY & STARFORMING & composite &  \\
 \hline
\multirow{2}{*}{137} & 1 & 1237655465916104829 & 0.132  & 18.21 & 17.28 & GALAXY & AGN & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237655465916104830 & 0.132  & 18.69 & 17.5  & GALAXY & ... & LINER &  \\
\hline
\multirow{2}{*}{138} & 1 & 1237653616938516591 & 0.099 & 17.12 & 16.19 & GALAXY & AGN & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237653616938516592 & 0.099 & 17.8 & 16.84  & GALAXY & ... & LINER &  \\
\hline
\multirow{2}{*}{139} & 1 & 1237652600635851575 & 0.175  & 18.06 & 17.01 & GALAXY & AGN & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237652600635851576 & 0.178 & 18.44 & 17.13 & GALAXY & ... & LINER &  \\
\hline
\multirow{2}{*}{140} & 1 & 1237651250968461337 & 0.223  & 18.82 & 18.39 & QSO & STARBURST & composite & \multirow{2}{*}{...} \\
 & 2 & 1237651250968461338 & 0.223 & 21.59 & 20.53 & GALAXY & STARBURST & composite &  \\
\hline
\multirow{2}{*}{141} & 1 & 1237648721245503520 & 0.047 & 17.75 & 17.16 & GALAXY & STARBURST & composite & \multirow{2}{*}{...} \\
 & 2 & 1237648721245503521 & 0.048  & 16.32 & 15.52 & GALAXY & AGN & seyfert &  \\
\hline
\multirow{2}{*}{142} & 1 & 1237648722312888376 & 0.138 & 17.81 & 17.16 & GALAXY & STARBURST & seyfert & \multirow{2}{*}{...} \\
 & 2 & 1237648722312888377 & 0.138 & 17.9 & 17.08 & GALAXY & AGN & seyfert &  \\
\hline
\multirow{2}{*}{143} & 1 & 1237654382514471111 & 0.06  & 16.93 & 16.18 & GALAXY & AGN & seyfert & \multirow{2}{*}{...} \\
 & 2 & 1237654382514471112 & 0.06 & 17.83 & 17.05  & GALAXY & STARFORMING & composite &  \\
\hline
\multirow{2}{*}{144} & 1 & 1237657191979286606 & 0.087 & 17.09 & 16.06 & QSO & STARBURST & seyfert & \multirow{2}{*}{...} \\
 & 2 & 1237657191979286607 & 0.087 & 17.28 & 16.35  & GALAXY & ... & LINER &  \\
\hline
\\
\\
\hline
\multirow{2}{*}{145} & 1 & 1237659326018355482 & 0.105 & 17.67 & 16.7 & GALAXY & ... & seyfert & \multirow{2}{*}{...} \\
 & 2 & 1237659326018355483 & 0.107 & 18.54 & 17.54 & GALAXY & AGN & seyfert &  \\
\hline
\multirow{2}{*}{146} & 1 & 1237661465992626516 & 0.063 & 17.53 & 16.54 & GALAXY & BROADLINE & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237661465992626517 & 0.065 & 17.24 & 16.22  & GALAXY & AGN & LINER &  \\
\hline
\multirow{2}{*}{147} & 1 & 1237661812275347597 & 0.091  & 17.72 & 16.87 & GALAXY & AGN & seyfert & \multirow{2}{*}{...} \\
 & 2 & 1237661812275347598 & 0.092  & 18.67 & 17.72 & GALAXY & ... & composite &  \\
\hline
\multirow{2}{*}{148} & 1 & 1237661813885436021 & 0.065  & 17.04 & 16.11 & GALAXY & ... & LINER & \multirow{2}{*}{...} \\
 & 2 & 1237661813885436022 & 0.065 & 17.62 & 16.79 & GALAXY & AGN & seyfert &  \\
\hline
\multirow{2}{*}{149} & 1 & 1237662224058089529 & 0.087 & 17.6 & 16.6 & GALAXY & ... & composite & \multirow{2}{*}{...} \\
 & 2 & 1237662224058024149 & 0.088  & 17.72 & 16.77 & GALAXY & AGN & LINER &  \\
\hline
\multirow{2}{*}{150} & 1 & 1237663542609117199 & 0.128 & 18.59 & 17.38 & QSO & STARBURST & seyfert & \multirow{2}{*}{...} \\
 & 2 & 1237663542609117200 & 0.128  & 18.23 & 17.11  & GALAXY & ... & composite &  \\
 \hline
 \multirow{3}{*}{151} & 1 & 1237661064950710579 & 0.126 & 17.12 & 16.03 & GALAXY & ... & composite & \multirow{3}{*}{\parbox{\linewidth}%
{Third source have insufficient  Line emission data}} \\
 & 2 & 1237661064950710580 & 0.125  & 17.75 & 16.71 & GALAXY & ... & LINER &  \\
 & 3 & 1237661064950710581 & 0.127 & 19.92 & 18.91  & GALAXY & ... & ... &  \\
 \hline
\multirow{3}{*}{152} & 1 & 1237663275777392799 & 0.094 & 19.14 & 18.1  & GALAXY & ... & composite & \multirow{3}{*}{\parbox{\linewidth}%
{Dual AGN with an associated SF nuclei}} \\
 & 2 & 1237663275777392800 & 0.095 & 17.14 & 16.13 & GALAXY & ... & seyfert &  \\
 & 3 & 1237663275777392798 & 0.091 & 18.57 & 17.53 & GALAXY & ... & SF &  \\
\hline
\multirow{3}{*}{153} & 1 & 1237663542608920721 & 0.144  & 18.8 & 17.59 & GALAXY & ... & LINER & \multirow{3}{*}{\parbox{\linewidth}%
{Dual AGN with an associated SF nuclei}} \\
 & 2 & 1237663542608920724 & 0.144 & 21.45 & 20.2 & GALAXY & ... & seyfert &  \\
 & 3 & 1237663542608920720 & 0.144 & 19.02 & 17.82 & GALAXY & ... & SF &  \\
 \hline
\multirow{3}{*}{154} & 1 & 1237663783126237343 & 0.063 & 17.49 & 16.54 & GALAXY & ... & composite & \multirow{3}{*}{\parbox{\linewidth}%
{Dual AGN with associated SF nuclei}} \\
 & 2 & 1237663783126237344 & 0.064 & 17.41 & 16.44 & GALAXY & ... & LINER &  \\
 & 3 & 1237663783126237342 & 0.064 & 16.26 & 15.34 & GALAXY & ... & SF &  \\
 \hline
\multirow{3}{*}{155} & 1 & 1237665564997714246 & 0.26 & 19.69 & 18.18 & GALAXY & ... & LINER & \multirow{3}{*}{\parbox{\linewidth}%
{Third source have insufficient Line emission data}} \\
 & 2 & 1237665564997779740 & 0.254 & 18.33 & 16.69 & GALAXY & ... & composite &  \\
 & 3 & 1237665564997714249 & 0.254 & 19.71 & 18.2 & GALAXY & ... & ... &  \\
 \hline
\multirow{3}{*}{156} & 1 & 1237668299280089194 & 0.063  & 16.34 & 15.41  & GALAXY & ... & LINER & \multirow{3}{*}{\parbox{\linewidth}%
{Third source have insufficient Line emission data}} \\
 & 2 & 1237668299280089196 & 0.063 & 17.68 & 16.93 & GALAXY & STARFORMING & composite &  \\
 & 3 & 1237668299280089195 & 0.062 & 16.64 & 15.73  & GALAXY & ... & ... &  \\
\hline
\multirow{4}{*}{157} & 1 & 1237666301093675376 & 0.086 & 17.55 & 16.76 & QSO & BROADLINE & LINER & \multirow{4}{*}{\parbox{\linewidth}%
{Dual AGN with 2 associated SF nuclei}} \\
 & 2 & 1237666301093675377 & 0.087 & 19.04 & 18.27 & GALAXY & ... & LINER &  \\
 & 3 & 1237666301093675378 & 0.088 & 18.5 & 17.87 & GALAXY & STARBURST & SF &  \\
 & 4 & 1237666301093675379 & 0.086 & 19.47 & 18.99 & GALAXY & STARFORMING & SF &  \\
 \hline
\multirow{3}{*}{158} & 1 & 1237657192517926989 & 0.105 & 18.33 & 17.34 & GALAXY & ... & LINER &  \multirow{3}{*}{Triple AGN} \\
 & 2 & 1237657192517926990 & 0.106 & 19.83 & 18.94 & GALAXY & ... & LINER &  \\
 & 3 & 1237657192517926993 & 0.106 & 17.87 & 16.88 & GALAXY & ... & seyfert &  \\
\hline
 \multirow{3}{*}{159}& 1 & 1237667736133107729 & 0.102  & 17.07 & 16.05 & GALAXY & ... & seyfert & \multirow{3}{*}{Triple AGN} \\ 
 & 2 & 1237667736133107730 & 0.103 & 17.02 & 15.96 & GALAXY & ... & LINER &  \\
 & 3 & 1237667736133107731 & 0.103 & 17.8 & 16.84 & GALAXY & BROADLINE & ... &  \\

 \hline                              
\end{longtable}

==> Tables/subsetdng.tex <==
\begin{table*}
\centering
\caption{Subset of the final reduced sample of double/multiple nuclei in closely interacting galaxies}
\begin{tabular}{lcccccccccccc}

\hline
No.  & Comp. &        Object        & Redshift & u     & g     & r    & i & z & M$_R$ & Class & Sublclass & Class\\
        &    No. &         id           &     z    &       &       &      &   &   &       &  SDSS & SDSS & BPT\\
\hline
\hline
\multirow{2}{*}{1}   & 1         & 1237645942905700478 & 0.131 & 20.84 & 18.74 & 17.44 & 16.78 & 16.34 & -22.6459 & GALAXY & ... & composite          \\
                     & 2         & 1237645942905700479 & 0.131 & 21.9  & 19.44 & 18.09 & 17.62 & 17.06 & -21.7872 & GALAXY & ... & ...          \\
                     \hline
\multirow{2}{*}{2} &  1    & 1237660636002713767 & 0.077 & 19.67 & 17.57 & 16.6  & 16.15 & 15.81 & -21.5264 & GALAXY & ... & SF          \\
                     &  2    & 1237660636002713768 & 0.079 & 19.61 & 17.47 & 16.48 & 16.01 & 15.7  & -21.8155 & GALAXY & AGN & composite        \\
                     \hline
\multirow{2}{*}{3} & 1 & 1237657191979286606 & 0.087 & 19.23 & 17.09 & 16.06 & 15.46 & 15.15 & -21.8744 & QSO & Starburst & seyfert \\
                     & 2    & 1237657191979286607 & 0.087 & 19.26 & 17.28 & 16.35 & 15.97 & 15.59 & -21.7874 & GALAXY & ... & LINER          \\
                     \hline
\multirow{2}{*}{4} &  1    & 1237661465992626516 & 0.063 & 19.53 & 17.53 & 16.54 & 16.08 & 15.72 & -21.6477 & GALAXY & Broadline & LINER    \\
                     & 2    & 1237661465992626517 & 0.065 & 19.36 & 17.24 & 16.22 & 15.72 & 15.36 & -21.6509 & GALAXY & AGN & LINER        \\
                     \hline
\multirow{2}{*}{5} &  1    & 1237661972259537090 & 0.072 & 18.89 & 17.01 & 16.1  & 15.61 & 15.35 & -21.7777 & QSO & Starburst & seyfert \\
                     & 2    & 1237661972259537092 & 0.072 & 18.85 & 17.41 & 16.68 & 16.27 & 15.99 & -21.3021 & GALAXY & Starforming & SF        \\
                     \hline
\multirow{2}{*}{6} &  1    & 1237662224066740430 & 0.107 & 20.19 & 18.16 & 17.28 & 16.83 & 16.49 & -20.5664 & GALAXY & AGN & composite        \\
                     & 2    & 1237662224066740431 & 0.107 & 19.04 & 18.06 & 17.76 & 17.48 & 17.4  & -20.0496 & GALAXY & Starburst & SF        \\
                     \hline
\multirow{2}{*}{7} &  1    & 1237659133284843796 & 0.269 & 19.54 & 19.06 & 18.16 & 17.74 & 17.36 & -22.9486 & QSO & Broadline & SF     \\
                    &  2    & 1237659133284843797 & 0.27  & 23.49 & 20.56 & 18.74 & 18.03 & 17.6  & -23.4795 & GALAXY & ... & LINER          \\
                     \hline
\multirow{2}{*}{8} &  1    & 1237651250968461337 & 0.223 & 18.97 & 18.82 & 18.39 & 18.01 & 17.98 & -21.3989 & QSO & Starburst & composite  \\
                     &  2    & 1237651250968461338 & 0.223 & 24.15 & 21.59 & 20.53 & 19.98 & 19.69 & -20.8064 & GALAXY & Starburst & composite        \\
                     \hline
\multirow{3}{*}{9} &  1    & 1237670965918957796 & 0.213 & 21.48 & 19.66 & 18.15 & 17.62 & 17.27 & -22.642  & GALAXY & ... & seyfert          \\
                     &  2    & 1237670965918957793 & 0.208 & 19.55 & 19.1  & 18.38 & 17.97 & 17.85 & -21.6676 & QSO & Starburst & SF  \\
                     &  3    & 1237670965918957798 & 0.212 & 24.18 & 19.65 & 18.26 & 17.65 & 17.31 & -22.1665 & GALAXY & ... & ...          \\
                     \hline
\multirow{4}{*}{10} &  1    & 1237663783680802920 & 0.025 & 21.26 & 20.88 & 20.82 & 20.83 & 20.91 & -19.9634 & G & ... & ...         \\
                     &  2    & 1237663783680802925 & 0.025 & 22.57 & 21.8  & 22.38 & 22.24 & 22.83 & -16.276  & GSB & ... & ...        \\
                     &  3    & 1237663783680802912 & 0.025 & 16.65 & 15.68 & 15.17 & 15.04 & 15.28 & -19.9353 & GSB & ... & ...        \\
                     &  4    & 1237663783680802915 & 0.025 & 20.8  & 20.3  & 20.59 & 20.76 & 21.9  & -19.5298 & GSB & ... & ...         \\
                     \hline

\label{table:reduced.subset}                                 \end{tabular}
\end{table*}
